How Good Are LLMs for Literary Translation, Really? Literary Translation Evaluation with Humans and LLMs

Recent research has focused on literary machine translation (MT) as a new challenge in MT. However, the evaluation of literary MT remains an open problem. We contribute to this ongoing discussion by introducing LITEVAL-CORPUS, a paragraph-level parallel corpus containing verified human translations and outputs from 9 MT systems, which totals over 2k translations and 13k evaluated sentences across four language pairs, costing 4.5k C. This corpus enables us to (i) examine the consistency and adequacy of human evaluation schemes with various degrees of complexity, (ii) compare evaluations by students and professionals, assess the effectiveness of (iii) LLM-based metrics and (iv) LLMs themselves. Our findings indicate that the adequacy of human evaluation is controlled by two factors: the complexity of the evaluation scheme (more complex is less adequate) and the expertise of evaluators (higher expertise yields more adequate evaluations). For instance, MQM (Multidimensional Quality Metrics), a complex scheme and the de facto standard for non-literary human MT evaluation, is largely inadequate for literary translation evaluation: with student evaluators, nearly 60% of human translations are misjudged as indistinguishable or inferior to machine translations. In contrast, BWS (BEST-WORST SCALING), a much simpler scheme, identifies human translations at a rate of 80-100%. Automatic metrics fare dramatically worse, with rates of at most 20%. Our overall evaluation indicates that published human translations consistently outperform LLM translations, where even the most recent LLMs tend to produce considerably more literal and less diverse translations compared to humans.

==> latex/tables/annotation_scheme.tex <==
\begin{table}\centering
\scriptsize
\begin{tabular}{llcc}\toprule
\multirow{2}{*}{Scheme} &\multirow{2}{*}{Detail} &\multicolumn{2}{c}{Evaluators} \\\cmidrule{3-4}
& &Student &Professional \\\midrule
\makecell[l]{\textbf{Free annotation} \\ (Span-level)} & \makecell[l]{(1) highlight error spans; \\(2) provide explanations} & &X \\
\arrayrulecolor{black! 5}\midrule
\makecell[l]{\textbf{MQM} \\ (Span-level)} &\makecell[l]{(1) highlight error spans;\\(2) categorize error type;\\(3) select error severity }&X & \\
\arrayrulecolor{black! 20}\midrule
\textbf{SQM} &scale rating &X &X \\
\arrayrulecolor{black! 20}\midrule
\makecell[l]{\textbf{Best-worst} \\(Top systems)} &direct comparison &X & \\
\arrayrulecolor{black! 100}\bottomrule
\end{tabular}
\caption{Summary of annotation schemes.}\label{tab:anno_scheme}
\end{table}

==> latex/tables/prof_annotation.tex <==
\begin{table}[H]\centering
\scriptsize
\begin{tabular}{lccccccc}\toprule
\multirow{2}{*}{Pair} &\multicolumn{2}{c}{SQM} & &\multicolumn{2}{c}{\makecell{Error span \\(span match)}} &\multirow{2}{*}{\#instance} \\\cmidrule{2-3}\cmidrule{5-6}
&S-S &S-P & &S-S &S-P & & \\\midrule
\deen &0.528 &0.363 & &0.282 &0.252 &20 \\
\enDe &0.151 &0.196 & &0.442 &0.318  &26 \\
\enzh &0.359 &0.517 & &0.374 &0.297 &22 \\
\dezh &\multicolumn{6}{c}{-} \\
Mean &0.346 &0.359 & &0.366 &0.289  & -\\
\bottomrule
\end{tabular}
\caption{Annotation agreement between pairs of two
student evaluators (S-S) and between student and professional translators (S-P). The agreement for SQM
score is measured by Kendall’s Tau; The span-level
comparison is measured by Cohen’s kappa, where span
match reflects the agreement on error spans.}\label{tab:agre_stupro}
\end{table}
